Potential and sky coverage for off-axis fringe tracking in optical long baseline interferometry

The spectacular results provided by the second-generation VLTI instruments GRAVITY and MATISSE on active galactic nuclei (AGN) trigger and justify a strong increase in the sensitivity limit of optical interferometers. A key component of such an upgrade is off-axis fringe tracking. To evaluate its potential and limitations, we describe and analyse its error budget including fringe sensing precision and temporal, angular and chromatic perturbations of the piston. The global tracking error is computed using standard seeing parameters for different sites, seeing conditions and telescope sizes for the current GRAVITY Fringe Tracker (GFT) and a new concept of Hierarchical Fringe Tracker. Then, it is combined with a large catalogue of guide star candidates from Gaia to produce sky coverage maps that give the probability to find a usable off-axis guide star in any part of the observable sky. These maps can be used to set the specifications of the system, check its sensitivity to seeing conditions, and evaluate the feasibility of science programs. We check the availability of guide stars and the tracking accuracy for a large set of 15 799 Quasars to confirm the feasibility of a large program on Broad Line Regions in the K band with the GFT and show how it can be extended to the L, M, and N bands. Another set of 331 well-characterized nearby AGNs shows the high potential of MATISSE for imaging and characterization of the dust torus in the N band under off-axis tracking on both Unit Telescopes and Auxiliary Telescopes.

==> 1-autors.tex <==
% The list of authors, and the short list which is used in the headers.
% If you need two or more lines of authors, add an extra line using \newauthor
\author[A. Boskri et al.]{
Abdelkarim Boskri,$^{1,2}$\thanks{E-mail:abdelkarim.boskri@ced.uca.ac.ma}
Romain G. Petrov,$^{2}$
Thami El Halkouj,$^{1}$
Massinissa Hadjara,$^{3,4,5}$
James Leftley$^{2}$
\newauthor
Zouhair  Benkhaldoun,$^{1}$
Pierre Cruzalèbes,$^{2}$
Aziz Ziad,$^{2}$
Marcel Carbillet,$^{2}$
\\
% List of institutions
$^{1}$LPHEA Laboratry, Oukaimeden Observatory, Cadi Ayyad University/FSSM, BP 2390, Marrakesh, Morocco\\
$^{2}$Université de la Côte d’Azur, Observatoire de la Côte d’Azur, CNRS, Laboratoire Lagrange, Parc Valrose, Bât. H. Fizeau, 06108 Nice, France\\
$^{3}$Chinese Academy of Sciences South America Center for Astronomy, National Astronomical Observatories, CAS, Beijing 100101, China\\
$^{4}$Departamento de Astronomía, Universidad de Chile, Casilla 36-D, Santiago, Chile\\
$^{5}$Centre de Recherche en Astronomie, Astrophysique et Géophysique (CRAAG), Route de l’Observatoire, B.P. 63, Bouzareah, 16340, Alger, Algeria
}


==> table.tex <==
\begin{table}\texttt{}
	\centering
\begin{tabular}{p{2.5cm}|p{1.cm}|p{0.9cm}|p{0.9cm}|p{0.9cm}|}
\cline{2-5}
\multirow{2}{*}{}                                 & \multicolumn{2}{c|}{GFT}  & GFT+     & HFT      \\ \cline{2-5} 
                                                  & ATs       & UTs           & UTs      & UTs      \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Nbr. telescopes NT}          & 4         & 4             & 4        & 4        \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Nbr. pairs NP}               & 3         & 3             & 3        & 1        \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Nbr. pixels}                 & 4         & 4             & 4        & 4        \\ \hline
\multicolumn{1}{|l|}{Nbr. spectral channels}      & 6         & 6             & 6        & 1        \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Spectral band Phase Delay}   & K         & K             & K        & H+Ks     \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Spectral band Group Delay}   & K         & K             & K        & J        \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Detector}                    & \multicolumn{4}{c|}{SAPHIRA}                    \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Read out noise D}            & \multicolumn{4}{c|}{0.7}                        \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Noise amplification}         & \multicolumn{4}{c|}{1.5}                        \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Transmission}                & 1\%       & 1\%           & 1\%      & 2\%      \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Photons/s  (K=0, Str=1}      & 6 107     & 1.2 108       & 1.2 108  &          \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Strehl in K}                 & 0.5       & \multicolumn{3}{c|}{0.6 (LGS mode)} \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Strehl in H}                 &           &               &          & 0.4      \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Strehl in J}                 &           &               &          & 0.2      \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Vibration residual V}        & 100       & 200           & 100      & 100      \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Atmospheric residual T}      & 200       & 200           & 200      & 200      \\ \hline
\multicolumn{1}{|p{2.5cm}|}{VI=exp-2(V2+T2)2}            & 0.81      & 0.69          & 0.81     & 0.75     \\ \hline
\multicolumn{1}{|p{2.5cm}|}{VE=1-2}                      & $\sim$1   & $\sim$0.16    & $\sim$1  & $\sim$1  \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Baseline}                    & G1-J3     & UT1-UT4       & UT1-UT4  & UT1-UT4  \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Seeing at 0.5 µm}            & \multicolumn{4}{c|}{0.6 arcsec}                 \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Coherence time at 0.5 µm}    & \multicolumn{4}{c|}{7 ms}                       \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Isoplanetic angle at 0.5 µm} & \multicolumn{4}{c|}{2.6 arcsec}                 \\ \hline
\multicolumn{1}{|p{2.5cm}|}{Outer Scale}                 & \multicolumn{4}{c|}{25 m}                       \\ \hline
\end{tabular}
\caption{Fringe Tracking parameters at Paranal Observatory}
\end{table}

